Efficient Global Occupancy Mapping for Mobile Robots using OpenVDB

In this work we present a fast occupancy map building approach based on the VDB datastructure. Existing log-odds based occupancy mapping systems are often not able to keep up with the high point densities and framerates of modern sensors. Therefore, we suggest a highly optimized approach based on a modern datastructure coming from a computer graphic background. A multithreaded insertion scheme allows occupancy map building at unprecedented speed. Multiple optimizations allow for a customizable tradeoff between runtime and map quality. We first demonstrate the effectiveness of the approach quantitatively on a set of ablation studies and typical benchmark sets, before we practically demonstrate the system using a legged robot and a UAV.

==> img/parallel.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.6\columnwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          scale=0.6,
          xlabel={Threads},
          ylabel={Runtime in [ms]},
          ylabel shift = -5 pt,
          xmin=0, xmax=12,
          ymin=0, ymax=50000,
          xtick={1,2,4,8,12},
          ymode=log,
          log basis y={10},
          legend pos=north east,
          ymajorgrids=true,
          grid style=dashed,
          ]
          \addplot[
          color=blue,
          mark=square,
          ]
          coordinates {
              (1,1131)(2,566)(4,253)(8,157)(12,132)
            };
          \legend{$\text{ray}_{6}$}
          \addplot[
          color=red,
          mark=triangle,
          ]
          coordinates {
              (1,12685)(2,9311)(4,8944)(8,11049)(12,13856)
            };
          \legend{$\text{ray}_{6}$, $\text{ray}_{60}$}
        \end{axis}
      \end{tikzpicture}
      \label{fig:eval_par}
  \end{subfigure}
  % \hfill
  \begin{subfigure}[b]{0.6\columnwidth}
    \centering
    \begin{tikzpicture}[
    every axis/.style={ % add these settings to all the axis environments in the tikzpicture
        scale=0.6,
        xmode=log,
        ymode=log,
        xtick={6, 12, 30, 60, 100},
        xlabel={Maximum range in [m]},
        ylabel={Runtime in [ms]},
        y domain=0:60000
        ytick={100, 1000, 10000, 50000},
        bar width=5pt,
        log x ticks with fixed point,
        % log y ticks with fixed point,
    },]
    \begin{axis}[legend pos=north west, legend cell align={left}, legend style={row sep=0pt, column sep=5pt}]
      \addlegendimage{only marks, mark=square*, blue};
      \addlegendimage{only marks, mark=square*, red};
      \addlegendimage{only marks, mark=square*, yellow};
      \addlegendimage{only marks, mark=star};

      \addlegendentry{\scriptsize{par-insert}}
      \addplot [fill=blue!70, bar shift=0pt, ybar stacked] coordinates {(6,10) (12,30) (30,136) (60,361) (100, 803)};
      \addlegendentry{\scriptsize{par-merge}}
      \addplot [fill=red!70, bar shift=0pt, ybar stacked] coordinates {(6,8) (12,47) (30,881) (60,6085) (100,24405)};
      \addlegendentry{\scriptsize{par-integrate}}
      \addplot [fill=yellow!70, bar shift=0pt, ybar stacked] coordinates {(6,3) (12,29) (30,393) (60,1943) (100,5801)};
      \addlegendentry{\scriptsize{normal}}
      \addplot +[] coordinates {(6,135) (12,379) (30,1269) (60,4631) (100, 12780)};
    \end{axis}

    \end{tikzpicture}
    \label{fig:eval_par1}
  \end{subfigure}
  \caption{Parallel insertion Performance.}
  \label{fig:map_integration_parallel}
\end{figure}

